Graph Homomorphisms for Quantum Players

A homomorphism from a graph $X$ to a graph $Y$ is an adjacency preserving mapping $f:V(X) \rightarrow V(Y)$. We consider a nonlocal game in which Alice and Bob are trying to convince a verifier with certainty that a graph $X$ admits a homomorphism to $Y$. This is a generalization of the well-studied graph coloring game. Via systematic study of quantum homomorphisms we prove new results for graph coloring. Most importantly, we show that the Lov\'{a}sz theta number of the complement lower bounds the quantum chromatic number, which itself is not known to be computable. We also show that some of our newly introduced graph parameters, namely quantum independence and clique numbers, can differ from their classical counterparts while others, namely quantum odd girth, cannot. Finally, we show that quantum homomorphisms closely relate to zero-error channel capacity. In particular, we use quantum homomorphisms to construct graphs for which entanglement-assistance increases their one-shot zero-error capacity.

==> Diagram.tex <==
%\documentclass{article}
%\usepackage{tikz}
%\usetikzlibrary{arrows}
%\begin{document}

\begin{tikzpicture}
[vx/.style = {inner sep = 3pt, text height=1.5ex,text depth=.25ex}];

\def\hstep{-1};
\def\wstep{1.5};
\def\wstepn{1.1};


\foreach \i/\name in
         {1/$\chi$,2/$\chi_q$,3/$\xi_f$,4/$\bar{\vartheta}$,
          5/$\;\,\bar{\Theta}^*$, 8/$\omega$}{
 \node[vx](\i) at (0,\i*\hstep) {\name};}

\node[vx](2l) at (-1*\wstep,2*\hstep) {$\chi_f$};
\node[vx](2r) at (\wstep,2*\hstep) {$\xi$};
\node[vx](6l) at (-1*\wstepn,6*\hstep) {$\bar{c}_0^*$};
\node[vx](7l) at (-1*\wstepn,7*\hstep) {$\omega_q$};
\node[vx](65r) at (\wstepn,6.5*\hstep) {$\bar{\Theta}$};



\draw (1) -- (2) -- (3) -- (4);
\draw (1) -- (2l) -- (3);
\draw (1) -- (2r) -- (3);
\draw[dashed] (4) -- (5);
\draw (5) -- (6l);
\draw[dashed] (6l) -- (7l);
\draw (7l) -- (8);
\draw (5) -- (65r) -- (8);


\node[rectangle,minimum height=15pt, minimum width=60pt, 
      rounded corners=7pt,draw=black!40](rect) 
at (0.5*\wstep,2*\hstep) {};

\end{tikzpicture}

%\end{document}


==> Prelim.tex <==
% !TEX root = Paper - JCTB.tex

In this paper graphs will be undirected and, unless explicitly defined otherwise, finite. A graph is said to be vertex/edge transitive if for any two vertices/edges, there exists an automorphism of the graph that maps one to the other. We will refer to orthogonal projectors (matrices which are both idempotent and Hermitian) simply as projectors. We say that two positive semidefinite matrices $E$ and $F$ of the same dimensions, are orthogonal if $EF=0$ or equivalently if $\tr(EF)=0$. Note that this also implies that the column spaces of $E$ and $F$ are orthogonal.
We use $\mathbb{M}_{\mathbb{F}}(m,n)$ to denote the space of $m\times n$ matrices over the field $\mathbb{F}$. For a matrix $M\in\mathbb{M}_{\mathbb{C}}(m,n)$, we write $\overline{M}$ to denote the $m\times n$ matrix obtained by taking the complex conjugate of each of the entries of $M$. Finally, for a natural number $n\ge 1$ we use $[n]$ to denote the set $\{1,\dotsc,n\}$.

\paragraph{Quantum states and measurements.}
We now briefly introduce the mathematical formalism used to describe quantum states and measurements. For an in-depth explanation we refer the reader to~\cite{NC}.

To any quantum system S, we associate a complex vector space $\mathbb{C}^d$ equipped with the usual inner product. A state of the system S can be specified by a unit vector $\psi\in\mathbb{C}^d$ or alternatively using a rank-one projection $\psi\psi^*$. These are the most basic type of quantum states and they are known as  pure states.
Now suppose that the quantum system S is prepared in state $\psi\in\mathbb{C}^d$ with probability $p$ and in state $\phi\in\mathbb{C}^d$ with probability  $1-p$. If we do not know which case has happened, we describe the state of S using the positive semidefinite matrix $p \psi\psi^* + (1-p)\phi\phi^*$. Such states are known as mixed states. More formally, a mixed state of system S is a positive semidefinite matrix $\rho\in\mathbb{M}_{\mathbb{C}}(d,d)$ with trace equal to one. We can extract classical information from a quantum system by measuring it. In this paper we describe a measurement using a positive-operator valued measure (POVM) and we thus use the terms ``measurement'' and ``POVM'' interchangeably. A POVM $\mathcal{E}$ is specified by a set $\{E_1,\ldots,E_n\}\subset\mathbb{M}_{\mathbb{C}}(d,d)$ of positive semidefinite operators such that $\sum_{i \in [n]} E_i = I_d$, where $I_d$ is the $d\times d$ identity matrix. A POVM, or measurement, is projective if each $E_i$ is a projector. Note that we can only measure a quantum system S using a measurement $\mathcal{E}$ if the dimension of the vector space associated to S matches the size of the matrices specifying the measurement $\mathcal{E}$. 
According to the axioms of quantum mechanics, if we measure a quantum system S in a mixed state $\rho$ using measurement $\mathcal{E}$, then we obtain outcome $i\in [n]$ with probability equal to $p_i = \tr(\rho E_i)$. In the case when the state $\rho$ is pure, i.e., $\rho = \psi\psi^*$, we can also express the probability $p_i$ as~$\psi^* E_i \psi$. 

Consider two quantum systems $\text{A}$ and $\text{B}$ with associated spaces $\mathbb{C}^{d_A}$ and $\mathbb{C}^{d_B}$ respectively. The vector space we associate to the combined quantum system $(\text{A},\text{B})$ is $\mathbb{C}^{d_A}\otimes \mathbb{C}^{d_B}$. Furthermore, if $\text{A}$ is in a state $\psi_1\in\mathbb{C}^{d_A}$ and $\text{B}$ is in state $\psi_2\in\mathbb{C}^{d_B}$, then their joint state is described using the tensor product $\psi_1\otimes\psi_2$. However, not all pure states of $(\text{A},\text{B})$ are tensor products. In fact, one of the key features of quantum mechanics, the phenomenon of entanglement, occurs when the state of the constituent quantum systems cannot be described independently. More precisely, a state $\psi\in\mathbb{C}^{d_A}\otimes \mathbb{C}^{d_B}$ is said to be entangled, if there does not exist a pair of states $\psi_1\in\mathbb{C}^{d_A}, \psi_2\in\mathbb{C}^{d_B}$ such that $\psi = \psi_1\otimes\psi_2$. We say that a quantum state $\psi \in \mathbb{C}^d \otimes \mathbb{C}^d$ is \emph{maximally entangled} if $\psi = \frac{1}{\sqrt{d}}\sum_{i = 1}^d u_i \otimes v_i$, where $\{u_1,\ldots,u_d\}$ and $\{v_1,\ldots,v_d\}$ are some orthonormal bases for $\mathbb{C}^d$. The \emph{canonical maximally entangled state} in $\mathbb{C}^d \otimes \mathbb{C}^d$ is 
\begin{equation}
  \Phi := \frac{1}{\sqrt{d}}\sum_{i=1}^d e_i \otimes e_i,
\end{equation}
where $e_i$ is the $i^\text{th}$ standard basis vector. 

Finally, let us discuss partial measurements of a composite quantum system $(\text{A},\text{B})$. If a POVM $\mathcal{E} = \{E_1,\dotsc,E_n\}$ can be used to measure system A then it can also be used to measure the A part of the composite system $(\text{A},\text{B})$. Applying $\mathcal{E}$ to a state $\psi\in\mathbb{C}^{d_A}\otimes \mathbb{C}^{d_B}$ of $(\text{A},\text{B})$ will yield outcome $i\in[n]$ with probability
\begin{equation}
  p_i = \psi^* (E_i \otimes I) \psi
\end{equation} 
leaving system B in state $\rho_i = \tfrac{1}{p_i} \tr_A((E_i \otimes I) \psi\psi^*)$. Here, $\tr_A: \mathbb{M}_{\mathbb{C}}(d_Ad_B,d_Ad_B) \to \mathbb{M}_{\mathbb{C}}(d_B,d_B)$ is the map defined by $\tr_A(M\otimes N) =\tr(M)N$ and extended linearity; this map is known as partial trace. We sometimes refer to the $\rho_i$ as the residual states. Note that there is no need to define residual states, when $p_i=0$ as this corresponds to a zero-probability event. To treat both the $p_i=0$ and the $p_i\ne 0$ case in a unified manner, it is sometimes convenient to consider the unnormalized residual states $\rho'_i := \tr_A((E_i \otimes I) \psi\psi^*)$. Note that the states $\rho'_i$ are well-defined and equal to the zero matrix for $p_i=0$. We stress that unnormalized states are used for convenience only and all quantum states are by definition normalized, i.e., of unit norm.

